Labor market conditions and college graduation: evidence from Brazil

College students graduating in a recession have been shown to face large and persistent negative effects on their earnings, health, and other outcomes. This paper investigates whether students delay graduation to avoid these effects. Using data on the universe of students in higher education in Brazil and leveraging variation in labor market conditions across time, space, and chosen majors, the paper finds that students in public institutions delay graduation to avoid entering depressed labor markets. A typical recession causes the on-time graduation rate to fall by 6.5% in public universities and there is no effect on private institutions. The induced delaying increases average graduation by 0.11 semesters, consistent with 1 out of 18 students delaying graduation by one year in public universities. The delaying effect is larger for students with higher scores, in higher-earnings majors, and from more advantaged backgrounds. This has important implications for the distributional impact of recessions.

==> FigTables/ufba_credits.tex <==
\begin{table}[!ht]
    \caption{UFBA --- Credits completed (IV) }\label{res:ufba_credits}
\begin{adjustbox}{max width = \textwidth, width = .7\textwidth, center}
\begin{threeparttable}
\begin{tabular}[t]{lccc}
      \hline \hline \\[-.2cm]
      & First Stage & Second Stage \\
       \cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3}
\emph{Outcome}  & \emph{On-time graduation} & \emph{Credits Completed} \\ 
\midrule
Hiring & -0.245\\
(s.e.) & (0.058)\\

\{F-stat\} & \{17.867\}\\
\\
On-time graduation && \num{-220.3} \\
 (s.e.) && (\num{331.6}) \\
 
 [p-value] && {}[\num{0.508}] \\
\\
N Obs & {20,206} & {20,206} \\
\hline \hline 
      \end{tabular}
\begin{tablenotes}
\item \footnotesize{Notes: The table presents the two stage least squares estimates for the effectts of on-time graduaiton on the number of credits obtained by graduates. I instrument the on-time graduation by the major-weighted hiring measure. In the first column we can see the first stage estimate (point estimate, standard errors and the F-statitistic). The second columns shows the second stage estimates. Standard errors are clustered at the major level. All regressions include fixed effects for program, time of admission, fall semester, and demographic cells (gender, race and age).}
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}


==> FigTables/ufba_credits_before.tex <==
\begin{table}[ht!]
    \caption{UFBA --- Credits obtained before graduation }\label{res:ufba_credits_before}
\begin{adjustbox}{max width = \textwidth, width = .9\textwidth, center}
\begin{threeparttable}
\begin{tabular}[t]{lccccc}
      \hline \hline \\[-.2cm]
      \multicolumn{1}{r}{\emph{Outcome:}} & \multicolumn{5}{c}{\emph{Credits Obtained}}\\
      \addlinespace 
Semesters before expected graduation:&  5 & 4 & 3 & 2 & 1 \\  
\midrule
Hiring x 1st T & \num{13.704} & \num{-33.940} & \num{-63.994} & \num{-88.143} & \num{20.258}\\
 (s.e.)& (\num{10.485}) & (\num{54.134}) & (\num{66.991}) & (\num{80.308}) & (\num{119.263})\\
 
 [p-value]& {}[\num{0.194}] & {}[\num{0.532}] & {}[\num{0.342}] & {}[\num{0.275}] & {}[\num{0.865}]\\
 \\
 Hiring x 2nd T & \num{42.736} & \num{62.531} & \num{-26.726} & \num{-77.691} & \num{-102.736}\\
 (s.e.)& (\num{35.096}) & (\num{35.366}) & (\num{76.511}) & (\num{62.047}) & (\num{101.729})\\
 
 [p-value]& {}[\num{0.226}] & {}[\num{0.080}] & {}[\num{0.728}] & {}[\num{0.214}] & {}[\num{0.315}]\\
\\
 Hiring x 3rd T & \num{39.303} & \num{98.585} & \num{-17.948} & \num{-93.984} & \num{-149.203}\\
 (s.e.)& (\num{34.327}) & (\num{40.891}) & (\num{59.259}) & (\num{51.829}) & (\num{103.254})\\
 
 [p-value]& {}[\num{0.255}] & {}[\num{0.018}] & {}[\num{0.763}] & {}[\num{0.073}] & {}[\num{0.152}]\\
\\
N Obs & {32,507} & {34,635} & {35,868} & {36,487} & {36,487}\\
\hline \hline 
      \end{tabular}
\begin{tablenotes}
\item \footnotesize{Notes: The table presents the estimation of $\beta$ from equation \ref{res:main_results} interacted with an indicator for students admission score tercile (computed within program-year) for students in UFBA. I multiply the coefficient by minus one, therefore we can see the coefficients as a decrease of 100\% of the weighted hiring measure. The recession between 2014-2016 reduced the weighted hiring measure by 30\%. In each column the outcome variable is the total number of credits obtained in semester $\tau$ relative to expeced gradution, where $\tau\in[1,5]$. Standard errors are clusteres at both the major and state levels (\emph{two-way clustering}). All regressions include fixed effects for program, time of admission, fall semester, and demographic cells (gender, race and age).}
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}


==> FigTables/ufba_gpa.tex <==
\begin{table}[!ht]
    \caption{UFBA --- Heterogeneity by GPA }\label{res:ufba_gpa}
\begin{adjustbox}{max width = \textwidth, width = .6\textwidth, center}
\begin{threeparttable}
\begin{tabular}[t]{lcccc}
      \hline \hline  \addlinespace
      GPA quartile & 1st & 2nd & 3rd & 4th \\ \addlinespace
      \hline \addlinespace
Effects & \num{-0.010} & \num{-0.035} & \num{-0.035} & \num{-0.037}\\
 (s.e.) & (\num{0.013}) & (\num{0.015}) & (\num{0.019}) & (\num{0.018})\\
 
 [p-value] & {}[\num{0.440}] & {}[\num{0.020}] & {}[\num{0.076}] & {}[\num{0.043}]\\
 \addlinespace
\hline \hline 
      \end{tabular}
\begin{tablenotes}
\item \footnotesize{Notes: Table presents the results for the interaction between GPA quartile and MSE in equation \ref{eq:main_specification}. Standard errors are clustered at the major level. I included fixed effects for program, time of admission, and demographics cells (gender, race, and age).}
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}

